The restricted isometry property meets nonlinear approximation with redundant frames

It is now well known that sparse or compressible vectors can be stably recovered from their low-dimensional projection, provided the projection matrix satisfies a Restricted Isometry Property (RIP). We establish new implications of the RIP with respect to nonlinear approximation in a Hilbert space with a redundant frame. The main ingredients of our approach are: a) Jackson and Bernstein inequalities, associated to the characterization of certain approximation spaces with interpolation spaces; b) a new proof that for overcomplete frames which satisfy a Bernstein inequality, these interpolation spaces are nothing but the collection of vectors admitting a representation in the dictionary with compressible coefficients; c) the proof that the RIP implies Bernstein inequalities. As a result, we obtain that in most overcomplete random Gaussian dictionaries with fixed aspect ratio, just as in any orthonormal basis, the error of best $m$-term approximation of a vector decays at a certain rate if, and only if, the vector admits a compressible expansion in the dictionary. Yet, for mildly overcomplete dictionaries with a one-dimensional kernel, we give examples where the Bernstein inequality holds, but the same inequality fails for even the smallest perturbation of the dictionary.

==> nearbestsparse.tex <==
\section{Near $\ell^\tau$ optimality of the $\ell^1$ minimizer ?}
\newcommand\sign[0]{\textrm{sign}}
We would like to find conditions on the dictionary $\dict$ so that the minimum $\ell^1$ norm solution to $f = \dict c$ is always guaranteed to be also a near best $\ell^\tau$ norm solution for a given $0<\tau\leq 1$.
Namely speaking, whenever
\[
c = \arg\min \|c\|_1\ \mbox{s.t.}\ f = \dict c
\]
for some $f$, we would like to also have
\begin{equation}
\label{eq:DefNearBestMin}
\|c\|_\tau^\tau \leq C \cdot \|c+v\|_\tau^\tau, \quad \forall z \in N(\dict).
\end{equation}
where $1 \leq C < \infty$. It will be convenient to write $C = \epsilon^{\tau-1}$ where $0<\epsilon\leq 1$.

A well-known necessary and sufficient condition for $c$ to be an $\ell^1$ minimizer is that $s: = \sign(c)$ satisfies
\begin{equation}
\label{eq:DefGoodSign}
|\langle s, z\rangle| \leq \|z_{\bar{\Lambda}}\|_1,\quad \forall z \in N(\dict),
\end{equation}
where $\bar{\Lambda}$ is the complement of the support $\lambda$ of $s$.

The property we are looking for is therefore that, for any $s$ satisfying~\eqref{eq:DefGoodSign}, and any $c$ such that $\sign(c) = s$,
\[
\|c_\lambda\|_\tau^\tau
 \leq \epsilon^{\tau-1} 
 \left\{
 \|c_\Lambda + z_\Lambda\right\|_\tau^\tau
 +
 \|z_{\bar{\Lambda}}\|_\tau^\tau
 \},
 \quad \forall z \in N(\dict).
\]
Equivalently, for any $s$ satisfying~\eqref{eq:DefGoodSign} and any $z \in N(\dict)$,
\begin{eqnarray*}
\|z_{\bar{\Lambda}}\|_\tau^\tau
&\geq&
\sup_{c | \sign(c) = s} 
\left\{
\epsilon^{1-\tau} \|c_\Lambda\|_\tau^\tau - \|c_\Lambda + z_\Lambda\|_\tau^\tau
\right\}\\
&=&
\sum_{k \in \Lambda}
\sup_{c_k | \sign(c_k) = s_k} \epsilon^{1-\tau} |c_k|^\tau-|c_k + z_k|^\tau\\
&=&
\sum_{k \in \Lambda}
\sup_{c> 0} \epsilon^{1-\tau}|c|^\tau- |c + s_k z_k|^\tau.
\end{eqnarray*}
Defining $f(c|a) := \epsilon^{1-\tau} c^\tau- |c+a|^\tau$ for $c>0$ and $a \in \mathbb{R}$, a simple function study shows that
\begin{itemize}
\item if $a<0$, then
\[
\sup_{c>0} f(c|a) = \max_{c>0} f(c|a) = \epsilon^{1-\tau}|a|^\tau;
\]
\item if $a\geq 0$, then
\[
\sup_{c>0} f(c|a) = \max_{c>0} f(c|a) = -(1-\epsilon)^{1-\tau} \cdot |a|^\tau
\]
\end{itemize}
Denoting $\Lambda^+(s,z) := \{ k \in \Lambda, s_k z_k > 0\}$ and $\Lambda^- (s,z) := \{k \in \Lambda, s_k z_k < 0\}$ (for shortness of notation we will drop the dependency of the sets $\Lambda^\pm$ on $s$, $z$ when possible), the desired property is: for any $s$ satisfying~\eqref{eq:DefGoodSign} and any $z \in N(\dict)$, 
\[
\|z_{\bar{\Lambda}}\|_\tau^\tau 
\geq
\epsilon^{1-\tau}\|z_{\Lambda^-}\|_\tau^\tau - (1-\epsilon)^{1-\tau} \|z_{\Lambda^+}\|_\tau^\tau.
\]
For $z \in N(\dict)$, denoting $\tilde{z} = -z \in N(\dict)$, we have $\Lambda^+(s,\tilde{z}) = \Lambda^-(s,z)$ and $\Lambda^-(s,\tilde{z}) = \Lambda^+(s,z)$, hence this is equivalent to: for $s$ as in~\eqref{eq:DefGoodSign} and $z \in N(\dict)$
\begin{equation*}
\|z_{\bar{\Lambda}}\|_\tau^\tau 
\geq
\epsilon^{1-\tau} \cdot
\max\left(\|z_{\Lambda^-}\|_\tau^\tau,\|z_{\Lambda^+}\|_\tau^\tau\right)
 - (1-\epsilon)^{1-\tau} \cdot
\min\left(\|z_{\Lambda^+}\|_\tau^\tau,\|z_{\Lambda^-}\|_\tau^\tau\right).
\end{equation*}
Adding $\|z_{\Lambda^+}\|_\tau^\tau + \|z_{\Lambda^-}\|_\tau^\tau$ on both sides this becomes: for all $z \in N(\dict)$
%\begin{eqnarray}
%\label{eq:DefCond1}
%\|z\|_\tau^\tau &\geq &
%[1+\epsilon^{1-\tau}] \cdot \|z_{\Lambda^+}\|_\tau^\tau
%+
%[1-(1-\epsilon)^{1-\tau}] \cdot \|z_{\Lambda^-}\|_\tau^\tau\\
%\label{eq:DefCond2}
%\|z\|_\tau^\tau &\geq &
%[1+\epsilon^{1-\tau}] \cdot \|z_{\Lambda^-}\|_\tau^\tau
%+
%[1-(1-\epsilon)^{1-\tau}] \cdot \|z_{\Lambda^+}\|_\tau^\tau
%\end{eqnarray}
\begin{equation}
\label{eq:DefCondLtau}
\|z\|_\tau^\tau \geq 
[1+\epsilon^{1-\tau}] \cdot 
\max\left(\|z_{\Lambda^-}\|_\tau^\tau,\|z_{\Lambda^+}\|_\tau^\tau\right)
+
[1-(1-\epsilon)^{1-\tau}] \cdot 
\min\left(\|z_{\Lambda^-}\|_\tau^\tau,\|z_{\Lambda^+}\|_\tau^\tau\right).
\end{equation}
Specializing to $\tau=1$ yields a property equivalent to~\eqref{eq:DefGoodSign}: for all $z \in N(\dict)$
\begin{equation}
\|z\|_1 \geq 2 \cdot \max \left(\|z_{\Lambda^+}\|_1, \|z_{\Lambda^-}\|_1\right).
\end{equation}


\begin{prop}
The unique $\ell^1$ minimizer $c$ is guaranteed to be a near best $\ell^\tau$ minimizer in the sense of~\eqref{eq:DefNearBestMin} if, and only if,
for every sign pattern $s$, whenever 
\begin{equation}
\label{eq:DefCondL1}
\max\left(\|z_{\Lambda^+(s,z)}\|_1, \|z_{\Lambda^-(s,z)}\|_1\right)
\leq
\|z\|_1/2,
\quad \forall z \in N(\dict),
\end{equation}
we also have~\eqref{eq:DefCondLtau} (for a well chosen $\epsilon$) for all $z \in N(\dict)$. 
\end{prop}

The example below is intended to illustrate that there are overcomplete dictionaries in arbitrarily high dimensions where such a guarantee holds for any $\tau < 1$, with a constant $\epsilon$ that depends on $\tau$ but remains bounded from infinity even when the dimension of the underlying space grows to infinity.
\begin{example}
Consider the example of a dictionary made of the Dirac basis and the DC Fourier vector in dimension $m$. The null space is spanned by the vector $z = (1,\ldots,1,-\sqrt{m}) \in \mathbb{R}^{m+1}$. 
\begin{itemize}
\item Case 1: consider a sign pattern $s$ which support does not contain the final entry. Let $k = \sharp \Lambda^+$ and $\ell = \sharp \Lambda^-$, which must satisfy $k + \ell \leq m$. Without loss of generality we assume $k \leq \ell$. On the one hand, \eqref{eq:DefCondL1} holds iff $\ell \leq (\sqrt{m} + m)/2$.
On the other hand,~\eqref{eq:DefCondLtau} holds iff
\[
[1+\epsilon^{1-\tau}] \cdot \ell
+
[1-(1-\epsilon)^{1-\tau}] \cdot k
\leq m+m^{\tau/2}.
\]
The maximum of the left hand side in the domain where $k+\ell \leq m$, $k \leq \ell$, $\ell \leq (m+\sqrt m)/2$ is achieved when the two boundary conditions $k+\ell \leq m$ and $\ell \leq (m+\sqrt{m})/2$ are both satistied. For simplicity assume that $m = p^2$ is a perfect square: the maximum is achieved when $\ell = (p^2+p)/2$ and $k = m-\ell = (p^2-p)/2$. Thus~\eqref{eq:DefCondLtau} holds iff
\[
[1+\epsilon^{1-\tau}]\cdot \frac{p^2+p}2 
+
[1-(1-\epsilon)^{1-\tau}]\cdot \frac{p^2-p}2 
\leq
p^2 + p^\tau 
\]
that is to say
%\[
%\epsilon^{1-\tau}\cdot \frac{p^2+p}2 
%-(1-\epsilon)^{1-\tau}\cdot \frac{p^2-p}2 
%\leq
%p^\tau 
%\]
\[
\epsilon^{1-\tau}\cdot (p+1)
-(1-\epsilon)^{1-\tau}\cdot (p-1) 
\leq
2p^{\tau-1} 
\]
A sufficient condition is
\[
\epsilon^{1-\tau}\cdot (p+1)
-(1-\epsilon)^{1-\tau}\cdot (p-1) 
\leq
\epsilon^{1-\tau}2p^{\tau-1} 
\]
which is equivalent to
\[
\epsilon^{1-\tau}\cdot (p+1-2p^{\tau-1}) \leq
(1-\epsilon)^{1-\tau}\cdot (p-1) 
\]
It is sufficient that
\[
\left(\frac{1-\epsilon}{\epsilon}\right)^{1-\tau} \geq
1+2\frac{1-p^{\tau-1}}{p-1}
\]
That is to say
\[
\epsilon \leq \frac{1}{1+\left(1+2\frac{1-p^{\tau-1}}{p-1}\right)^{1/(1-\tau)}}
\]
It holds for any $\epsilon < 1/2$, as soon as $p$ is large enough.
\item Case 2: consider a sign pattern $s$ which support intersects the final entry. Without loss of generality assume that the final entry is in $\Lambda^+$. On the one hand~\eqref{eq:DefCondL1} holds iff $\sqrt{m}+(k-1) \leq (m+\sqrt{m})/2$ and $\ell \leq  (m+\sqrt{m})/2$ implying that
\[
\max(m^{\tau/2}+k-1,\ell) \leq (m+\sqrt{m})/2
\]
\[
\min(m^{\tau/2}+k-1,\ell) \leq (m+2m^{\tau/2}-\sqrt{m})/2
\]
On the other hand,~\eqref{eq:DefCondLtau} holds iff
\begin{eqnarray*}
&& [1+\epsilon^{1-\tau}] \cdot \max( m^{\tau/2} + k-1, \ell) \\
&&+ [1- (1-\epsilon)^{1-\tau}] \cdot \min (m^{\tau/2}+k-1,\ell) 
\leq m^{\tau/2} + m. 
\end{eqnarray*}
When~\eqref{eq:DefCondL1} holds, the left hand side is bounded from above by
\begin{eqnarray*}
&&[1+\epsilon^{1-\tau}] \cdot (m+\sqrt m)/2\\
&& + [1- (1-\epsilon)^{1-\tau}] (m+2m^{\tau/2}-\sqrt m)/2 \\
&\leq& m^{\tau/2} + m 
+
\epsilon^{1-\tau} (m+\sqrt m)/2 - (1-\epsilon)^{1-\tau} (m+2m^{\tau/2}-\sqrt m)/2
\end{eqnarray*}
hence~\eqref{eq:DefCondLtau} is guaranteed to hold as soon as
\[
\epsilon^{1-\tau} (m+\sqrt m) - (1-\epsilon)^{1-\tau} (m+2m^{\tau/2}-\sqrt m) \leq 0
\]
that is to say
\[
\left(\frac{1-\epsilon}{\epsilon}\right)^{1-\tau} \geq \frac{m+\sqrt m}{m+2m^{\tau/2}-\sqrt m}
=\frac{p^2+p}{p^2+2p^\tau -p} = \frac{p+1}{p+1 +2(p^{\tau-1}-1)}
\]
\end{itemize}
This example shows that for certain dictionaries it is indeed possible to find $\epsilon$ so that the desired property holds {\em even for large dimension $m$}, illustrating in a sense that the constant $C$, which depends on $\tau$, does not depend on the dimension.
\end{example}

The next question is whether the desired guarantee can also hold for more general dictionaries with null space of higher dimension, and whether a Bernstein inequality and/or RIP is sufficient to have the desired guarantee.
